Monoidal computer I: Basic computability by string diagrams

We present a new model of computation, described in terms of monoidal categories. It conforms the Church-Turing Thesis, and captures the same computable functions as the standard models. It provides a succinct categorical interface to most of them, free of their diverse implementation details, using the ideas and structures that in the meantime emerged from research in semantics of computation and programming. The salient feature of the language of monoidal categories is that it is supported by a sound and complete graphical formalism, string diagrams, which provide a concrete and intuitive interface for abstract reasoning about computation. The original motivation and the ultimate goal of this effort is to provide a convenient high level programming language for a theory of computational resources, such as one-way functions, and trapdoor functions, by adopting the methods for hiding the low level implementation details that emerged from practice. In the present paper, we make a first step towards this ambitious goal, and sketch a path to reach it. This path is pursued in three sequel papers, that are in preparation.

==> PIC/NNO-mult.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 11:37:58 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="66.26" y-min="-2.5" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,16.88);(8.12,16.88);(28.75,28.75);(28.75,28.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(58.75,30);(58.75,30);(41.25,30);(41.25,30)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(58.75,0);(58.75,0);(41.25,0);(41.25,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(35,26.88);(35,26.88);(35,4.38);(35,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(65,26.88);(65,26.88);(65,4.38);(65,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,23.75)"
%	 text-rotation= "25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,5.62)"
%	 text-rotation= "-25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(36.26,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.26,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,13.12);(8.12,13.12);(28.75,1.88);(28.75,1.88)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.26,32.5)
\rput(5,15){$\Lhh$}
\rput(35,30){$\UpOne$}
\rput(65,30){$\UpTwo$}
\rput(35,0){$\DownOne$}
\psline{->}(8.12,16.88)(28.75,28.75)
\psline{->}(58.75,30)(41.25,30)
\psline{->}(58.75,0)(41.25,0)
\psline[linestyle=dashed,dash=1 1]{->}(35,26.88)(35,4.38)
\psline[linestyle=dashed,dash=1 1]{->}(65,26.88)(65,4.38)
\rput(65,0){$\DownTwo$}
\rput{25}(16.25,23.75){$\one$}
\rput{-25}(16.88,5.62){$\two$}
\rput(50,32.5){$\three$}
\rput(50,-2.5){$\four$}
\rput[l](36.26,15.62){$\five$}
\rput[l](66.26,15.62){$\six$}
\psline{->}(8.12,13.12)(28.75,1.88)
\end{pspicture}


==> PIC/NNO-neg.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jul 07 15:20:11 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="66.25" y-min="-1.25" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,16.88);(8.12,16.88);(31.88,28.12);(31.88,28.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.88,30);(61.88,30);(39.38,30);(39.38,30)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(48.12,0);(48.12,0);(38.75,0);(38.75,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(35,26.88);(35,26.88);(35,4.38);(35,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(65,26.88);(65,26.88);(65,4.38);(65,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,23.75)"
%	 text-rotation= "25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,5.62)"
%	 text-rotation= "-25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(43.75,-0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35.62,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.25,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,13.12);(8.12,13.12);(31.88,1.25);(31.88,1.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,0);(61.25,0);(51.88,0);(51.88,0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$I$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(56.25,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\seven$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.25,32.5)
\rput(5,15){$\Lhh$}
\rput(35,30){$\UpOne$}
\rput(65,30){$\UpTwo$}
\rput(35,0){$\DownOne$}
\psline{->}(8.12,16.88)(31.88,28.12)
\psline{->}(61.88,30)(39.38,30)
\psline{->}(48.12,0)(38.75,0)
\psline[linestyle=dashed,dash=1 1]{->}(35,26.88)(35,4.38)
\psline[linestyle=dashed,dash=1 1]{->}(65,26.88)(65,4.38)
\rput(65,0){$\DownTwo$}
\rput{25}(16.25,23.75){$\one$}
\rput{-25}(16.88,5.62){$\two$}
\rput(50,32.5){$\three$}
\rput[t](43.75,-0.62){$\four$}
\rput[l](35.62,15.62){$\five$}
\rput[l](66.25,15.62){$\six$}
\psline{->}(8.12,13.12)(31.88,1.25)
\psline{->}(61.25,0)(51.88,0)
\rput(50,0){$I$}
\rput[t](56.25,-1.25){$\seven$}
\end{pspicture}


==> PIC/NNO-pred.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 16:20:35 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="66.25" y-min="-2.5" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,30)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,16.88);(8.12,16.88);(32.5,28.75);(32.5,28.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.88,30);(61.88,30);(38.75,30);(38.75,30)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(56.88,0);(56.88,0);(42.5,0);(42.5,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(35,26.88);(35,26.88);(35,4.38);(35,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 stroke-dasharray= "1;1"
%	 stroke-style= "dashed"
%	 points= "(65,26.88);(65,26.88);(65,4.38);(65,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.25,23.75)"
%	 text-rotation= "25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,5.62)"
%	 text-rotation= "-25"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(50,32.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(48.75,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35.62,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(66.25,15.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\six$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,13.12);(8.12,13.12);(28.12,2.5);(28.12,2.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(66.25,32.5)
\rput(5,15){$\Lhh$}
\rput(35,30){$\UpOne$}
\rput(65,30){$\UpTwo$}
\rput(35,0){$\DownOne$}
\psline{->}(8.12,16.88)(32.5,28.75)
\psline{->}(61.88,30)(38.75,30)
\psline{->}(56.88,0)(42.5,0)
\psline[linestyle=dashed,dash=1 1]{->}(35,26.88)(35,4.38)
\psline[linestyle=dashed,dash=1 1]{->}(65,26.88)(65,4.38)
\rput(65,0){$\DownTwo$}
\rput{25}(16.25,23.75){$\one$}
\rput{-25}(16.88,5.62){$\two$}
\rput(50,32.5){$\three$}
\rput(48.75,-2.5){$\four$}
\rput[l](35.62,15.62){$\five$}
\rput[l](66.25,15.62){$\six$}
\psline{->}(8.12,13.12)(28.12,2.5)
\end{pspicture}


==> PIC/OWF.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:06:48 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.62" x-max="18.26" y-min="-33.75" y-max="33.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(4.37,-21.76);(4.37,-21.76);(4.37,-16.26);(4.37,-16.26)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-21.76);(15,-21.76);(15,-16.26);(15,-16.26)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(7.13,-16.26)"
%	 p2= "(7.13,-10)"
%	 p1= "(1.63,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(2,-21.76);(2,-21.76);(18.26,-21.76);(18.26,-21.76);(18.26,-21.76);(13.26,-26.76);
%	(13.26,-26.76);(13.26,-26.76);(7,-26.76);(7,-26.76);(7,-26.76);(2,-21.76)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(18.12,22.5);(18.12,22.5);(1.88,22.5);(1.88,22.5);(1.88,22.5);(6.88,27.5);
%	(6.88,27.5);(6.88,27.5);(13.12,27.5);(13.12,27.5);(13.12,27.5);(18.12,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(9.99,27.5);(9.99,27.5);(9.99,33.13);(9.99,33.13)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(7.13,-3.12)"
%	 p2= "(7.13,3.12)"
%	 p1= "(1.63,3.12)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.74,-16.26)"
%	 p2= "(17.76,-10)"
%	 p1= "(12.25,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-10);(15,-10);(15,22.5);(15,22.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.37,3.12);(4.37,3.12);(4.37,9.38);(4.37,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(4.37,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(4.37,0.01)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(7.12,9.38)"
%	 p2= "(7.12,15.62)"
%	 p1= "(1.62,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,15.62);(4.38,15.62);(4.38,22.51);(4.38,22.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,-9.38);(4.38,-9.38);(4.38,-3.12);(4.38,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(4.38,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<multicurve fill-style= "none"
%	 points= "(9.99,-30.62);(9.99,-30.62);(9.99,-26.76);(9.99,-26.76)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(13.12,-30.62);(13.12,-30.62);(9.99,-33.75);(9.99,-33.75);(9.99,-33.75);(6.88,-30.62);
%	(6.88,-30.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.88,-30.62);(6.88,-30.62);(13.12,-30.62);(13.12,-30.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\indist$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(18.26,33.13)
\psline{->}(4.37,-21.76)(4.37,-16.26)
\psline{->}(15,-21.76)(15,-16.26)
\pspolygon[](1.63,-10)(7.13,-10)(7.13,-16.26)(1.63,-16.26)
\pspolygon(2,-21.76)
(18.26,-21.76)
(13.26,-26.76)
(7,-26.76)(2,-21.76)
\pspolygon(18.12,22.5)
(1.88,22.5)
(6.88,27.5)
(13.12,27.5)(18.12,22.5)
\psline{->}(9.99,27.5)(9.99,33.13)
\pspolygon[](1.63,3.12)(7.13,3.12)(7.13,-3.12)(1.63,-3.12)
\pspolygon[](12.25,-10)(17.76,-10)(17.74,-16.26)(12.23,-16.26)
\psline{->}(15,-10)(15,22.5)
\psline{->}(4.37,3.12)(4.37,9.38)
\rput(4.37,-13.12){$\one$}
\rput(4.37,0.01){$\two$}
\rput(15,-13.12){$\four$}
\pspolygon[](1.62,15.62)(7.12,15.62)(7.12,9.38)(1.62,9.38)
\psline{->}(4.38,15.62)(4.38,22.51)
\psline{->}(4.38,-9.38)(4.38,-3.12)
\rput(4.38,12.5){$\three$}
\psline{->}(9.99,-30.62)(9.99,-26.76)
\psline[fillstyle=solid](13.12,-30.62)
(9.99,-33.75)(6.88,-30.62)
\psline(6.88,-30.62)(13.12,-30.62)
\rput(10,25){$\indist$}
\end{pspicture}


==> PIC/TDF-open.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:34:05 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="28.88" y-min="-33.75" y-max="33.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,-21.76);(15,-21.76);(15,-16.26);(15,-16.26)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-21.76);(25.62,-21.76);(25.62,-16.26);(25.62,-16.26)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-16.26)"
%	 p2= "(17.76,-10)"
%	 p1= "(12.25,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.62,-21.76);(12.62,-21.76);(28.88,-21.76);(28.88,-21.76);(28.88,-21.76);(23.88,-26.76);
%	(23.88,-26.76);(23.88,-26.76);(17.62,-26.76);(17.62,-26.76);(17.62,-26.76);(12.62,-21.76)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.74,22.5);(28.74,22.5);(12.5,22.5);(12.5,22.5);(12.5,22.5);(17.5,27.5);
%	(17.5,27.5);(17.5,27.5);(23.74,27.5);(23.74,27.5);(23.74,27.5);(28.74,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,27.5);(20.62,27.5);(20.62,33.13);(20.62,33.13)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-3.12)"
%	 p2= "(17.76,3.12)"
%	 p1= "(0,3.12)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(28.36,-16.26)"
%	 p2= "(28.38,-10)"
%	 p1= "(22.88,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-10);(25.62,-10);(25.62,22.5);(25.62,22.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,3.12);(15,3.12);(15,9.38);(15,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,0.01)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25.62,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(17.74,9.38)"
%	 p2= "(17.74,15.62)"
%	 p1= "(12.25,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15.62);(15,15.62);(15,22.51);(15,22.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-9.38);(15,-9.38);(15,-3.12);(15,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20.62,-30.62);(20.62,-30.62);(20.62,-26.76);(20.62,-26.76)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(23.74,-30.62);(23.74,-30.62);(20.62,-33.75);(20.62,-33.75);(20.62,-33.75);(17.5,-30.62);
%	(17.5,-30.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,-30.62);(17.5,-30.62);(23.74,-30.62);(23.74,-30.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20.62,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\indist$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.12,-6.87);(3.12,-6.87);(3.12,-3.01);(3.12,-3.01)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.24,-6.87);(6.24,-6.87);(3.12,-10);(3.12,-10);(3.12,-10);(0,-6.87);
%	(0,-6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-6.87);(0,-6.87);(6.24,-6.87);(6.24,-6.87)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(22.5,-33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\exx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,-8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eyy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28.88,33.13)
\psline{->}(15,-21.76)(15,-16.26)
\psline{->}(25.62,-21.76)(25.62,-16.26)
\pspolygon[](12.25,-10)(17.76,-10)(17.76,-16.26)(12.25,-16.26)
\pspolygon(12.62,-21.76)
(28.88,-21.76)
(23.88,-26.76)
(17.62,-26.76)(12.62,-21.76)
\pspolygon(28.74,22.5)
(12.5,22.5)
(17.5,27.5)
(23.74,27.5)(28.74,22.5)
\psline{->}(20.62,27.5)(20.62,33.13)
\pspolygon[](0,3.12)(17.76,3.12)(17.76,-3.12)(0,-3.12)
\pspolygon[](22.88,-10)(28.38,-10)(28.36,-16.26)(22.85,-16.26)
\psline{->}(25.62,-10)(25.62,22.5)
\psline{->}(15,3.12)(15,9.38)
\rput(15,-13.12){$\one$}
\rput(15,0.01){$\two$}
\rput(25.62,-13.12){$\four$}
\pspolygon[](12.25,15.62)(17.74,15.62)(17.74,9.38)(12.25,9.38)
\psline{->}(15,15.62)(15,22.51)
\psline{->}(15,-9.38)(15,-3.12)
\rput(15,12.5){$\three$}
\psline{->}(20.62,-30.62)(20.62,-26.76)
\psline[fillstyle=solid](23.74,-30.62)
(20.62,-33.75)(17.5,-30.62)
\psline(17.5,-30.62)(23.74,-30.62)
\rput(20.62,25){$\indist$}
\psline{->}(3.12,-6.87)(3.12,-3.01)
\psline(6.24,-6.87)
(3.12,-10)(0,-6.87)
\psline(0,-6.87)(6.24,-6.87)
\rput[tl](22.5,-33.12){$\exx$}
\rput(3.12,-8.12){$\eyy$}
\end{pspicture}


==> PIC/TDF.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:30:06 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="28.88" y-min="-33.75" y-max="33.13" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(15,-21.76);(15,-21.76);(15,-16.26);(15,-16.26)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-21.76);(25.62,-21.76);(25.62,-16.26);(25.62,-16.26)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-16.26)"
%	 p2= "(17.76,-10)"
%	 p1= "(12.25,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.62,-21.76);(12.62,-21.76);(28.88,-21.76);(28.88,-21.76);(28.88,-21.76);(23.88,-26.76);
%	(23.88,-26.76);(23.88,-26.76);(17.62,-26.76);(17.62,-26.76);(17.62,-26.76);(12.62,-21.76)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(28.74,22.5);(28.74,22.5);(12.5,22.5);(12.5,22.5);(12.5,22.5);(17.5,27.5);
%	(17.5,27.5);(17.5,27.5);(23.74,27.5);(23.74,27.5);(23.74,27.5);(28.74,22.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,27.5);(20.62,27.5);(20.62,33.13);(20.62,33.13)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(17.76,-3.12)"
%	 p2= "(17.76,3.12)"
%	 p1= "(0,3.12)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(28.36,-16.26)"
%	 p2= "(28.38,-10)"
%	 p1= "(22.88,-10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-10);(25.62,-10);(25.62,22.5);(25.62,22.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,3.12);(15,3.12);(15,9.38);(15,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,0.01)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(25.62,-13.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(17.74,9.38)"
%	 p2= "(17.74,15.62)"
%	 p1= "(12.25,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,15.62);(15,15.62);(15,22.51);(15,22.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(15,-9.38);(15,-9.38);(15,-3.12);(15,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<multicurve fill-style= "none"
%	 points= "(20.62,-30.62);(20.62,-30.62);(20.62,-26.76);(20.62,-26.76)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(23.74,-30.62);(23.74,-30.62);(20.62,-33.75);(20.62,-33.75);(20.62,-33.75);(17.5,-30.62);
%	(17.5,-30.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.5,-30.62);(17.5,-30.62);(23.74,-30.62);(23.74,-30.62)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20.62,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\indist$
%</text>
%<multicurve fill-style= "none"
%	 points= "(3.12,-6.87);(3.12,-6.87);(3.12,-3.01);(3.12,-3.01)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "solid"
%	 points= "(6.24,-6.87);(6.24,-6.87);(3.12,-10);(3.12,-10);(3.12,-10);(0,-6.87);
%	(0,-6.87)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,-6.87);(0,-6.87);(6.24,-6.87);(6.24,-6.87)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(22.5,-33.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\exx$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(1.25,-9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\eyy$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28.88,33.13)
\psline{->}(15,-21.76)(15,-16.26)
\psline{->}(25.62,-21.76)(25.62,-16.26)
\pspolygon[](12.25,-10)(17.76,-10)(17.76,-16.26)(12.25,-16.26)
\pspolygon(12.62,-21.76)
(28.88,-21.76)
(23.88,-26.76)
(17.62,-26.76)(12.62,-21.76)
\pspolygon(28.74,22.5)
(12.5,22.5)
(17.5,27.5)
(23.74,27.5)(28.74,22.5)
\psline{->}(20.62,27.5)(20.62,33.13)
\pspolygon[](0,3.12)(17.76,3.12)(17.76,-3.12)(0,-3.12)
\pspolygon[](22.88,-10)(28.38,-10)(28.36,-16.26)(22.85,-16.26)
\psline{->}(25.62,-10)(25.62,22.5)
\psline{->}(15,3.12)(15,9.38)
\rput(15,-13.12){$\one$}
\rput(15,0.01){$\two$}
\rput(25.62,-13.12){$\four$}
\pspolygon[](12.25,15.62)(17.74,15.62)(17.74,9.38)(12.25,9.38)
\psline{->}(15,15.62)(15,22.51)
\psline{->}(15,-9.38)(15,-3.12)
\rput(15,12.5){$\three$}
\psline{->}(20.62,-30.62)(20.62,-26.76)
\psline[fillstyle=solid](23.74,-30.62)
(20.62,-33.75)(17.5,-30.62)
\psline(17.5,-30.62)(23.74,-30.62)
\rput(20.62,25){$\indist$}
\psline{->}(3.12,-6.87)(3.12,-3.01)
\psline[fillstyle=solid](6.24,-6.87)
(3.12,-10)(0,-6.87)
\psline(0,-6.87)(6.24,-6.87)
\rput[tl](22.5,-33.12){$\exx$}
\rput[tr](1.25,-9.38){$\eyy$}
\end{pspicture}


==> PIC/abstraction.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 12:26:01 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.27" x-max="17.5" y-min="-12.5" y-max="11.88" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.75);(5,0.75)"
%	 />
%<parallelogram p3= "(17.5,-1.12)"
%	 p2= "(17.5,4.88)"
%	 fill-style= "none"
%	 p1= "(1.88,4.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,4.88);(5,4.88);(5,11.88);(5,11.88)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10.62,1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(6,0.75)"
%	 p2= "(6,2.75)"
%	 fill-style= "solid"
%	 p1= "(4,2.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.27,-6.25);(1.27,-6.25);(8.12,-6.25);(8.12,-6.25);(8.12,-6.25);(4.39,-12.5);
%	(4.39,-12.5);(4.39,-12.5);(1.27,-6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.5,11.88)
\psline{->}(5,-6.25)(5,0.75)
\pspolygon[](1.88,4.88)(17.5,4.88)(17.5,-1.12)(1.88,-1.12)
\psline{->}(5,4.88)(5,11.88)
\rput(10.62,1.88){$\ahh$}
\rput(5,-8.75){$\aah$}
\pspolygon[fillstyle=solid](4,2.75)(6,2.75)(6,0.75)(4,0.75)
\pspolygon(1.27,-6.25)
(8.12,-6.25)
(4.39,-12.5)(1.27,-6.25)
\end{pspicture}


==> PIC/application.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 13:10:23 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.27" x-max="20.49" y-min="-12.5" y-max="11.75" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.75);(5,0.75)"
%	 />
%<parallelogram p3= "(20,-1.25)"
%	 p2= "(20,4.75)"
%	 fill-style= "none"
%	 p1= "(2,4.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,4.75);(17,4.75);(17,11.75);(17,11.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(6,0.75)"
%	 p2= "(6,2.75)"
%	 fill-style= "solid"
%	 p1= "(4,2.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(16.88,-6.25);(16.88,-6.25);(16.88,-1.25);(16.88,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16.88,-8.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.27,-6.25);(1.27,-6.25);(8.12,-6.25);(8.12,-6.25);(8.12,-6.25);(4.39,-12.5);
%	(4.39,-12.5);(4.39,-12.5);(1.27,-6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.64,-6.25);(13.64,-6.25);(20.49,-6.25);(20.49,-6.25);(20.49,-6.25);(16.76,-12.5);
%	(16.76,-12.5);(16.76,-12.5);(13.64,-6.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20.49,11.75)
\psline{->}(5,-6.25)(5,0.75)
\pspolygon[](2,4.75)(20,4.75)(20,-1.25)(2,-1.25)
\psline{->}(17,4.75)(17,11.75)
\rput(13.12,1.88){$\ahh$}
\rput(5,-8.75){$\aah$}
\pspolygon[fillstyle=solid](4,2.75)(6,2.75)(6,0.75)(4,0.75)
\psline{->}(16.88,-6.25)(16.88,-1.25)
\rput(16.88,-8.75){$\bhh$}
\pspolygon(1.27,-6.25)
(8.12,-6.25)
(4.39,-12.5)(1.27,-6.25)
\pspolygon(13.64,-6.25)
(20.49,-6.25)
(16.76,-12.5)(13.64,-6.25)
\end{pspicture}


==> PIC/charfun.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 23:40:21 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="55.62" y-min="-17.5" y-max="16.88" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\One$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,-15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(55.62,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Five$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,11.88);(5,11.88);(5,-12.5);(5,-12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(35,11.88);(35,11.88);(35,-12.5);(35,-12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(9.38,15);(9.38,15);(31.88,15);(31.88,15)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.75,-15);(8.75,-15);(30.62,-15);(30.62,-15)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(37.5,13.12);(37.5,13.12);(51.25,2.5);(51.25,2.5)"
%	 />
%<multicurve left-arrow= "head"
%	 fill-style= "none"
%	 points= "(37.5,-12.5);(37.5,-12.5);(50,-1.25);(50,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.12,16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(18.75,-17.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(29.38,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(46.88,10)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(47.5,-9.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\five$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(55.62,16.88)
\rput(5,15){$\One$}
\rput(5,-15){$\Two$}
\rput(35,15){$\Three$}
\rput(35,-15){$\Four$}
\rput(55.62,0){$\Five$}
\psline{->}(5,11.88)(5,-12.5)
\psline{->}(35,11.88)(35,-12.5)
\psline{->}(9.38,15)(31.88,15)
\psline{->}(8.75,-15)(30.62,-15)
\psline{->}(37.5,13.12)(51.25,2.5)
\psline{<-}(37.5,-12.5)(50,-1.25)
\rput(18.12,16.88){$\one$}
\rput(18.75,-17.5){$\two$}
\rput(29.38,0){$\three$}
\rput(46.88,10){$\four$}
\rput(47.5,-9.38){$\five$}
\end{pspicture}


==> PIC/computation-wide.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 07:01:26 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="10.62" y-min="-10" y-max="10.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(5,-10);(5,-10);(5,-3.12);(5,-3.12)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(10.62,-3.12)"
%	 p2= "(10.62,3.75)"
%	 p1= "(-0.62,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,3.75);(5,3.75);(5,10.62);(5,10.62)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10.62,10.62)
\psline{->}(5,-10)(5,-3.12)
\rput(5,0){$\ahh$}
\pspolygon[](-0.62,3.75)(10.62,3.75)(10.62,-3.12)(-0.62,-3.12)
\psline{->}(5,3.75)(5,10.62)
\end{pspicture}


==> PIC/constant.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 17:12:20 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0" x-max="10" y-min="-11.25" y-max="11.88" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-11.25);(5,-11.25);(5,-5);(5,-5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,3.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,5);(5,5);(5,11.88);(5,11.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0,5);(0,5);(10,5);(10,5);(10,5);(5,0);
%	(5,0);(5,0);(0,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(10,-5);(10,-5);(-0,-5);(-0,-5);(-0,-5);(5,-0);
%	(5,-0);(5,-0);(10,-5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,11.88)
\psline{->}(5,-11.25)(5,-5)
\rput(5,-3.12){$\ahh$}
\rput(5,3.12){$\aah$}
\psline{->}(5,5)(5,11.88)
\pspolygon(0,5)
(10,5)
(5,0)(0,5)
\pspolygon(10,-5)
(-0,-5)
(5,-0)(10,-5)
\end{pspicture}


==> PIC/convolution-equality-P-down.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jul 16 10:47:33 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-16.88" y-max="35.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,-4.88);(3.12,-4.88);(3.12,0.62);(3.12,0.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,6.88);(3.12,6.88);(3.12,12.5);(3.12,12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,-4.88);(13.12,-4.88);(13.12,0.62);(13.12,0.62)"
%	 />
%<parallelogram p3= "(5.88,0.62)"
%	 p2= "(5.88,6.88)"
%	 fill-style= "none"
%	 p1= "(0.38,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,-4.88);(0.12,-4.88);(16.38,-4.88);(16.38,-4.88);(16.38,-4.88);(11.38,-9.88);
%	(11.38,-9.88);(11.38,-9.88);(5.12,-9.88);(5.12,-9.88);(5.12,-9.88);(0.12,-4.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-13.75);(8.12,-13.75);(8.12,-9.88);(8.12,-9.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,12.5);(16.25,12.5);(0,12.5);(0,12.5);(0,12.5);(5,17.5);
%	(5,17.5);(5,17.5);(11.25,17.5);(11.25,17.5);(11.25,17.5);(16.25,12.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,17.5);(8.12,17.5);(8.12,21.88);(8.12,21.88)"
%	 />
%<parallelogram p3= "(15.88,0.62)"
%	 p2= "(15.88,6.88)"
%	 fill-style= "none"
%	 p1= "(10.38,6.88)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,6.88);(13.12,6.88);(13.12,12.5);(13.12,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(3.12,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(13.12,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram p3= "(10.88,21.88)"
%	 p2= "(10.88,28.12)"
%	 fill-style= "none"
%	 p1= "(5.38,28.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,28.12);(8.12,28.12);(8.12,33.75);(8.12,33.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,-13.75);(11.25,-13.75);(8.12,-16.88);(8.12,-16.88);(8.12,-16.88);(5,-13.75);
%	(5,-13.75)"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(10,-16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,35.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,-13.75);(5,-13.75);(11.25,-13.75);(11.25,-13.75)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,35.62)
\psline{->}(3.12,-4.88)(3.12,0.62)
\psline{->}(3.12,6.88)(3.12,12.5)
\psline{->}(13.12,-4.88)(13.12,0.62)
\pspolygon[](0.38,6.88)(5.88,6.88)(5.88,0.62)(0.38,0.62)
\pspolygon(0.12,-4.88)
(16.38,-4.88)
(11.38,-9.88)
(5.12,-9.88)(0.12,-4.88)
\psline{->}(8.12,-13.75)(8.12,-9.88)
\pspolygon(16.25,12.5)
(0,12.5)
(5,17.5)
(11.25,17.5)(16.25,12.5)
\psline{->}(8.12,17.5)(8.12,21.88)
\pspolygon[](10.38,6.88)(15.88,6.88)(15.88,0.62)(10.38,0.62)
\psline{->}(13.12,6.88)(13.12,12.5)
\rput(3.12,3.75){$\one$}
\rput(13.12,3.75){$\two$}
\pspolygon[](5.38,28.12)(10.88,28.12)(10.88,21.88)(5.38,21.88)
\psline{->}(8.12,28.12)(8.12,33.75)
\psline(11.25,-13.75)
(8.12,-16.88)(5,-13.75)
\rput[tl](10,-16.25){$\variable$}
\rput(8.12,25){$\defnd$}
\rput(8.12,35.62){$\Lhh$}
\psline(5,-13.75)(11.25,-13.75)
\end{pspicture}


==> PIC/convolution-equality-P-tags.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 10:27:07 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="50.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,27.5);(3.12,27.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,15.62);(13.12,15.62)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,1.25);(8.12,1.25);(8.12,5.12);(8.12,5.12)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,27.5);(16.25,27.5);(0,27.5);(0,27.5);(0,27.5);(5,32.5);
%	(5,32.5);(5,32.5);(11.25,32.5);(11.25,32.5);(11.25,32.5);(16.25,27.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,32.5);(8.12,32.5);(8.12,36.88);(8.12,36.88)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(15.88,15.62)"
%	 p2= "(15.88,21.88)"
%	 p1= "(10.38,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,21.88);(13.12,21.88);(13.12,27.5);(13.12,27.5)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(10.88,36.88)"
%	 p2= "(10.88,43.12)"
%	 p1= "(5.38,43.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,43.12);(8.12,43.12);(8.12,48.75);(8.12,48.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,1.25);(11.25,1.25);(8.12,-1.88);(8.12,-1.88);(8.12,-1.88);(5,1.25);
%	(5,1.25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "top"
%	 anchor-point= "(10,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,40)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,50.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,1.25);(5,1.25);(11.25,1.25);(11.25,1.25)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,24.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Mu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(1.88,24.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Mu$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(1.88,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lu$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,50.62)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,27.5)
\psline{->}(13.12,10.12)(13.12,15.62)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,1.25)(8.12,5.12)
\pspolygon(16.25,27.5)
(0,27.5)
(5,32.5)
(11.25,32.5)(16.25,27.5)
\psline{->}(8.12,32.5)(8.12,36.88)
\pspolygon[](10.38,21.88)(15.88,21.88)(15.88,15.62)(10.38,15.62)
\psline{->}(13.12,21.88)(13.12,27.5)
\rput(3.12,18.75){$\one$}
\rput(13.12,18.75){$\two$}
\pspolygon[](5.38,43.12)(10.88,43.12)(10.88,36.88)(5.38,36.88)
\psline{->}(8.12,43.12)(8.12,48.75)
\psline(11.25,1.25)
(8.12,-1.88)(5,1.25)
\rput[tl](10,-1.25){$\variable$}
\rput(8.12,40){$\defnd$}
\rput(8.12,50.62){$\Lhh$}
\psline(5,1.25)(11.25,1.25)
\rput[l](13.75,24.38){$\Mu$}
\rput[l](13.75,12.5){$\Lu$}
\rput[r](1.88,24.38){$\Mu$}
\rput[r](1.88,12.5){$\Lu$}
\end{pspicture}


==> PIC/convolution-equality-P.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 18:04:49 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="50.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,27.5);(3.12,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,15.62);(13.12,15.62)"
%	 />
%<parallelogram p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,1.25);(8.12,1.25);(8.12,5.12);(8.12,5.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,27.5);(16.25,27.5);(0,27.5);(0,27.5);(0,27.5);(5,32.5);
%	(5,32.5);(5,32.5);(11.25,32.5);(11.25,32.5);(11.25,32.5);(16.25,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,32.5);(8.12,32.5);(8.12,36.88);(8.12,36.88)"
%	 />
%<parallelogram p3= "(15.88,15.62)"
%	 p2= "(15.88,21.88)"
%	 p1= "(10.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,21.88);(13.12,21.88);(13.12,27.5);(13.12,27.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram p3= "(10.88,36.88)"
%	 p2= "(10.88,43.12)"
%	 p1= "(5.38,43.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,43.12);(8.12,43.12);(8.12,48.75);(8.12,48.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(11.25,1.25);(11.25,1.25);(8.12,-1.88);(8.12,-1.88);(8.12,-1.88);(5,1.25);
%	(5,1.25)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(10,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,50.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,1.25);(5,1.25);(11.25,1.25);(11.25,1.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,50.62)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,27.5)
\psline{->}(13.12,10.12)(13.12,15.62)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,1.25)(8.12,5.12)
\pspolygon(16.25,27.5)
(0,27.5)
(5,32.5)
(11.25,32.5)(16.25,27.5)
\psline{->}(8.12,32.5)(8.12,36.88)
\pspolygon[](10.38,21.88)(15.88,21.88)(15.88,15.62)(10.38,15.62)
\psline{->}(13.12,21.88)(13.12,27.5)
\rput(3.12,18.75){$\one$}
\rput(13.12,18.75){$\two$}
\pspolygon[](5.38,43.12)(10.88,43.12)(10.88,36.88)(5.38,36.88)
\psline{->}(8.12,43.12)(8.12,48.75)
\psline(11.25,1.25)
(8.12,-1.88)(5,1.25)
\rput[tl](10,-1.25){$\variable$}
\rput(8.12,40){$\defnd$}
\rput(8.12,50.62){$\Lhh$}
\psline(5,1.25)(11.25,1.25)
\end{pspicture}


==> PIC/convolution-equality.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 17:42:50 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="50.62" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,27.5);(3.12,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,15.62);(13.12,15.62)"
%	 />
%<parallelogram p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-0.62);(8.12,-0.62);(8.12,5.12);(8.12,5.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,27.5);(16.25,27.5);(0,27.5);(0,27.5);(0,27.5);(5,32.5);
%	(5,32.5);(5,32.5);(11.25,32.5);(11.25,32.5);(11.25,32.5);(16.25,27.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,32.5);(8.12,32.5);(8.12,36.88);(8.12,36.88)"
%	 />
%<parallelogram p3= "(15.88,15.62)"
%	 p2= "(15.88,21.88)"
%	 p1= "(10.38,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,21.88);(13.12,21.88);(13.12,27.5);(13.12,27.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram p3= "(10.88,36.88)"
%	 p2= "(10.88,43.12)"
%	 p1= "(5.38,43.12)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,43.12);(8.12,43.12);(8.12,48.75);(8.12,48.75)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(11.25,1.25);(11.25,1.25);(8.12,-1.88);(8.12,-1.88);(8.12,-1.88);(5,1.25);
%	(5,1.25)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(10,-1.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\defnd$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,50.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,50.62)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,27.5)
\psline{->}(13.12,10.12)(13.12,15.62)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,-0.62)(8.12,5.12)
\pspolygon(16.25,27.5)
(0,27.5)
(5,32.5)
(11.25,32.5)(16.25,27.5)
\psline{->}(8.12,32.5)(8.12,36.88)
\pspolygon[](10.38,21.88)(15.88,21.88)(15.88,15.62)(10.38,15.62)
\psline{->}(13.12,21.88)(13.12,27.5)
\rput(3.12,18.75){$\one$}
\rput(13.12,18.75){$\two$}
\pspolygon[](5.38,43.12)(10.88,43.12)(10.88,36.88)(5.38,36.88)
\psline{->}(8.12,43.12)(8.12,48.75)
\psline[linewidth=0.05,fillstyle=solid](11.25,1.25)
(8.12,-1.88)(5,1.25)
\rput[tl](10,-1.25){$\variable$}
\rput(8.12,40){$\defnd$}
\rput(8.12,50.62){$\Lhh$}
\end{pspicture}


==> PIC/convolution-oper.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 07:09:27 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.12" x-max="25.12" y-min="-21.88" y-max="22.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(7.5,-8);(7.5,-8);(7.5,-2.51);(7.5,-2.51)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(7.5,3.75);(7.5,3.75);(7.5,9.38);(7.5,9.38)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.49,-8);(17.49,-8);(17.49,-2.51);(17.49,-2.51)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(10.25,-2.51)"
%	 p2= "(10.25,3.75)"
%	 p1= "(4.76,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.5,-8);(4.5,-8);(20.76,-8);(20.76,-8);(20.76,-8);(15.76,-13);
%	(15.76,-13);(15.76,-13);(9.5,-13);(9.5,-13);(9.5,-13);(4.5,-8)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,-21.88);(12.5,-21.88);(12.5,-13);(12.5,-13)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(20.62,9.38);(20.62,9.38);(4.38,9.38);(4.38,9.38);(4.38,9.38);(9.38,14.38);
%	(9.38,14.38);(9.38,14.38);(15.62,14.38);(15.62,14.38);(15.62,14.38);(20.62,9.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(12.5,14.38);(12.5,14.38);(12.5,22.5);(12.5,22.5)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(20.26,-2.51)"
%	 p2= "(20.26,3.75)"
%	 p1= "(14.76,3.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(17.49,3.75);(17.49,3.75);(17.49,9.38);(17.49,9.38)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(7.5,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(17.49,0.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<parallelogram fill-style= "none"
%	 p3= "(25.12,-17.5)"
%	 p2= "(25.12,17.5)"
%	 p1= "(-0.12,17.5)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "bottom"
%	 anchor-point= "(24.38,-16.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\ahh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(25.12,22.5)
\psline{->}(7.5,-8)(7.5,-2.51)
\psline{->}(7.5,3.75)(7.5,9.38)
\psline{->}(17.49,-8)(17.49,-2.51)
\pspolygon[](4.76,3.75)(10.25,3.75)(10.25,-2.51)(4.76,-2.51)
\pspolygon(4.5,-8)
(20.76,-8)
(15.76,-13)
(9.5,-13)(4.5,-8)
\psline{->}(12.5,-21.88)(12.5,-13)
\pspolygon(20.62,9.38)
(4.38,9.38)
(9.38,14.38)
(15.62,14.38)(20.62,9.38)
\psline{->}(12.5,14.38)(12.5,22.5)
\pspolygon[](14.76,3.75)(20.26,3.75)(20.26,-2.51)(14.76,-2.51)
\psline{->}(17.49,3.75)(17.49,9.38)
\rput(7.5,0.62){$\one$}
\rput(17.49,0.62){$\two$}
\pspolygon[](-0.12,17.5)(25.12,17.5)(25.12,-17.5)(-0.12,-17.5)
\rput[br](24.38,-16.88){$\ahh$}
\end{pspicture}


==> PIC/diag-comm <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 12 19:13:12 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="30" y-min="-2.5" y-max="16.25" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.49,2.5);(2.49,2.5);(13.75,13.75);(13.75,13.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,0);(3.75,0);(26.25,0);(26.25,0)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.88,9.38)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(23.12,9.38)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,13.75);(16.25,13.75);(27.5,2.5);(27.5,2.5)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(30,16.25)
\rput(0,0){$\Lhh$}
\rput(15,16.25){$\UpOne$}
\rput(30,0){$\DownOne$}
\psline{->}(2.49,2.5)(13.75,13.75)
\psline{->}(3.75,0)(26.25,0)
\rput{45}(6.88,9.38){$\one$}
\rput{-45}(23.12,9.38){$\two$}
\rput(13.75,-2.5){$\four$}
\psline{->}(16.25,13.75)(27.5,2.5)
\end{pspicture}


==> PIC/diag-comm.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 12 19:16:04 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="30" y-min="-2.5" y-max="16.25" auto-bounding="true">
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(15,16.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(30,0)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<multicurve fill-style= "none"
%	 points= "(2.49,2.5);(2.49,2.5);(13.75,13.75);(13.75,13.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,0);(3.75,0);(26.25,0);(26.25,0)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.88,9.38)"
%	 text-rotation= "45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(23.12,9.38)"
%	 text-rotation= "-45"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.75,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<multicurve fill-style= "none"
%	 points= "(16.25,13.75);(16.25,13.75);(27.5,2.5);(27.5,2.5)"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(30,16.25)
\rput(0,0){$\Lhh$}
\rput(15,16.25){$\UpOne$}
\rput(30,0){$\DownOne$}
\psline{->}(2.49,2.5)(13.75,13.75)
\psline{->}(3.75,0)(26.25,0)
\rput{45}(6.88,9.38){$\one$}
\rput{-45}(23.12,9.38){$\two$}
\rput(13.75,-2.5){$\four$}
\psline{->}(16.25,13.75)(27.5,2.5)
\end{pspicture}


==> PIC/diag-compreh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Jul 13 16:10:51 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.88" x-max="17.13" y-min="-3.12" y-max="67.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(14.37,10.12);(14.37,10.12);(14.37,15.62);(14.37,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(14.37,21.88);(14.37,21.88);(14.37,31.25);(14.37,31.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.87,10.12);(1.87,10.12);(1.88,15.62);(1.88,15.62)"
%	 />
%<parallelogram p3= "(17.13,15.62)"
%	 p2= "(17.13,21.88)"
%	 p1= "(11.63,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,0.12);(8.12,0.12);(8.12,5.12);(8.12,5.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,43.75);(16.25,43.75);(0,43.75);(0,43.75);(0,43.75);(5,48.75);
%	(5,48.75);(5,48.75);(11.25,48.75);(11.25,48.75);(11.25,48.75);(16.25,43.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,48.75);(8.12,48.75);(8.12,54.38);(8.12,54.38)"
%	 />
%<parallelogram p3= "(17.13,31.25)"
%	 p2= "(17.13,37.5)"
%	 p1= "(11.63,37.5)"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(4.62,15.62)"
%	 p2= "(4.63,21.88)"
%	 p1= "(-0.87,21.88)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(1.88,21.88);(1.88,21.88);(1.87,43.75);(1.87,43.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(14.37,37.5);(14.37,37.5);(14.37,43.75);(14.37,43.75)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(0.62,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15.62,26.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,63.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownOne$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.37,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.37,34.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<parallelogram p3= "(10.88,54.38)"
%	 p2= "(10.88,60.62)"
%	 p1= "(5.38,60.62)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,60.62);(8.12,60.62);(8.12,67.5);(8.12,67.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.38,51.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Lhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,-3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Xhh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(8.12,57.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\predicate$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(17.13,67.5)
\psline{->}(14.37,10.12)(14.37,15.62)
\psline{->}(14.37,21.88)(14.37,31.25)
\psline{->}(1.87,10.12)(1.88,15.62)
\pspolygon[](11.63,21.88)(17.13,21.88)(17.13,15.62)(11.63,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,0.12)(8.12,5.12)
\pspolygon(16.25,43.75)
(0,43.75)
(5,48.75)
(11.25,48.75)(16.25,43.75)
\psline{->}(8.12,48.75)(8.12,54.38)
\pspolygon[](11.63,37.5)(17.13,37.5)(17.13,31.25)(11.63,31.25)
\pspolygon[](-0.87,21.88)(4.63,21.88)(4.62,15.62)(-0.88,15.62)
\psline{->}(1.88,21.88)(1.87,43.75)
\psline{->}(14.37,37.5)(14.37,43.75)
\rput[r](0.62,32.5){$\Lhh$}
\rput[l](15.62,26.25){$\UpOne$}
\rput[l](9.38,63.75){$\DownOne$}
\rput(14.37,18.75){$\one$}
\rput(14.37,34.38){$\two$}
\rput(1.88,18.75){$\four$}
\pspolygon[](5.38,60.62)(10.88,60.62)(10.88,54.38)(5.38,54.38)
\psline{->}(8.12,60.62)(8.12,67.5)
\rput[l](9.38,51.25){$\Lhh$}
\rput(8.12,-3.12){$\Xhh$}
\rput(8.12,57.5){$\predicate$}
\end{pspicture}


==> PIC/diag-string.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 12 19:17:11 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.38" y-min="-1.88" y-max="58.12" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(3.12,10.12);(3.12,10.12);(3.12,15.62);(3.12,15.62)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,21.88);(3.12,21.88);(3.12,31.25);(3.12,31.25)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,10.12);(13.12,10.12);(13.12,23.75);(13.12,23.75)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(5.88,15.62)"
%	 p2= "(5.88,21.88)"
%	 p1= "(0.38,21.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(0.12,10.12);(0.12,10.12);(16.38,10.12);(16.38,10.12);(16.38,10.12);(11.38,5.12);
%	(11.38,5.12);(11.38,5.12);(5.12,5.12);(5.12,5.12);(5.12,5.12);(0.12,10.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,0.12);(8.12,0.12);(8.12,5.12);(8.12,5.12)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,43.75);(16.25,43.75);(0,43.75);(0,43.75);(0,43.75);(5,48.75);
%	(5,48.75);(5,48.75);(11.25,48.75);(11.25,48.75);(11.25,48.75);(16.25,43.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(8.12,48.75);(8.12,48.75);(8.12,55.75);(8.12,55.75)"
%	 right-arrow= "head"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(5.88,31.25)"
%	 p2= "(5.88,37.5)"
%	 p1= "(0.38,37.5)"
%	 />
%<parallelogram fill-style= "none"
%	 p3= "(15.88,23.75)"
%	 p2= "(15.88,30)"
%	 p1= "(10.38,30)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(13.12,30);(13.12,30);(13.12,43.75);(13.12,43.75)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.12,37.5);(3.12,37.5);(3.12,43.75);(3.12,43.75)"
%	 right-arrow= "head"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,-1.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Lhh$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(0.62,26.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\UpOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(8.12,58.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\DownOne$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,18.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(3.12,34.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(13.12,26.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.38,58.12)
\psline{->}(3.12,10.12)(3.12,15.62)
\psline{->}(3.12,21.88)(3.12,31.25)
\psline{->}(13.12,10.12)(13.12,23.75)
\pspolygon[](0.38,21.88)(5.88,21.88)(5.88,15.62)(0.38,15.62)
\pspolygon(0.12,10.12)
(16.38,10.12)
(11.38,5.12)
(5.12,5.12)(0.12,10.12)
\psline{->}(8.12,0.12)(8.12,5.12)
\pspolygon(16.25,43.75)
(0,43.75)
(5,48.75)
(11.25,48.75)(16.25,43.75)
\psline{->}(8.12,48.75)(8.12,55.75)
\pspolygon[](0.38,37.5)(5.88,37.5)(5.88,31.25)(0.38,31.25)
\pspolygon[](10.38,30)(15.88,30)(15.88,23.75)(10.38,23.75)
\psline{->}(13.12,30)(13.12,43.75)
\psline{->}(3.12,37.5)(3.12,43.75)
\rput(8.12,-1.88){$\Lhh$}
\rput(0.62,26.25){$\UpOne$}
\rput(8.12,58.12){$\DownOne$}
\rput(3.12,18.75){$\one$}
\rput(3.12,34.38){$\two$}
\rput(13.12,26.88){$\four$}
\end{pspicture}


==> PIC/ensemble-square.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 18 21:54:14 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="104.38" y-min="0" y-max="32.5" auto-bounding="true">
%<text text-vert-align= "top"
%	 anchor-point= "(1.88,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpOne$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpTwo$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(1.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(31.25,30);(31.25,30);(12,30);(12,30)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(31.25,0);(31.25,0);(12,0);(12,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.75,26.88);(3.75,26.88);(3.75,4.38);(3.75,4.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(33.75,26.88);(33.75,26.88);(33.75,4.38);(33.75,4.38)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownTwo$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(1.88,15.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\five$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.88,15.62)"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\six$
%</text>
%<multicurve left-arrow= "head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(101.25,30);(101.25,30);(90,30);(90,30)"
%	 />
%<multicurve left-arrow= "head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(101.25,0);(101.25,0);(89.38,0);(89.38,0)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(63.75,26.88);(63.75,26.88);(63.75,4.38);(63.75,4.38)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(61.88,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpThree$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(61.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownThree$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(62.5,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\seven$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(86,30);(86,30);(72,30);(72,30)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(86,0);(86,0);(72,0);(72,0)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,30);(61.25,30);(42,30);(42,30)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,0);(61.25,0);(42,0);(42,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(100.62,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\UpFour$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(101.25,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownFour$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(103.12,26.87);(103.12,26.87);(103.12,4.38);(103.12,4.38)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(104.38,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\eight$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(104.38,32.5)
\rput[tl](1.88,32.5){$\UpOne$}
\rput[tl](31.88,32.5){$\UpTwo$}
\rput[tl](1.88,2.5){$\DownOne$}
\psline{<-<}(31.25,30)(12,30)
\psline{<-<}(31.25,0)(12,0)
\psline{->}(3.75,26.88)(3.75,4.38)
\psline{->}(33.75,26.88)(33.75,4.38)
\rput[tl](31.88,2.5){$\DownTwo$}
\rput[r](1.88,15.62){$\five$}
\rput[r](31.88,15.62){$\six$}
\psline[linewidth=0.5,linestyle=dotted]{<-}(101.25,30)(90,30)
\psline[linewidth=0.5,linestyle=dotted]{<-}(101.25,0)(89.38,0)
\psline{->}(63.75,26.88)(63.75,4.38)
\rput[tl](61.88,32.5){$\UpThree$}
\rput[tl](61.88,2.5){$\DownThree$}
\rput[r](62.5,15){$\seven$}
\psline[linewidth=0.5,linestyle=dotted]{-<}(86,30)(72,30)
\psline[linewidth=0.5,linestyle=dotted]{-<}(86,0)(72,0)
\psline{<-<}(61.25,30)(42,30)
\psline{<-<}(61.25,0)(42,0)
\rput[tl](100.62,32.5){$\UpFour$}
\rput[tl](101.25,2.5){$\DownFour$}
\psline{->}(103.12,26.87)(103.12,4.38)
\rput[l](104.38,15){$\eight$}
\end{pspicture}


==> PIC/ensemble-tower.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 18 22:15:42 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.88" x-max="101.25" y-min="0" y-max="2.5" auto-bounding="true">
%<text text-vert-align= "top"
%	 anchor-point= "(1.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownOne$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(31.25,0);(31.25,0);(12,0);(12,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownTwo$
%</text>
%<multicurve left-arrow= "head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(101.25,0);(101.25,0);(89.38,0);(89.38,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(61.88,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownThree$
%</text>
%<multicurve right-arrow= "reverse-head"
%	 stroke-width= "0.5"
%	 fill-style= "none"
%	 stroke-style= "dotted"
%	 points= "(86,0);(86,0);(72,0);(72,0)"
%	 />
%<multicurve right-arrow= "reverse-head"
%	 left-arrow= "head"
%	 fill-style= "none"
%	 points= "(61.25,0);(61.25,0);(42,0);(42,0)"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(101.25,2.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\DownFour$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(101.25,2.5)
\rput[tl](1.88,2.5){$\DownOne$}
\psline{<-<}(31.25,0)(12,0)
\rput[tl](31.88,2.5){$\DownTwo$}
\psline[linewidth=0.5,linestyle=dotted]{<-}(101.25,0)(89.38,0)
\rput[tl](61.88,2.5){$\DownThree$}
\psline[linewidth=0.5,linestyle=dotted]{-<}(86,0)(72,0)
\psline{<-<}(61.25,0)(42,0)
\rput[tl](101.25,2.5){$\DownFour$}
\end{pspicture}


==> PIC/f.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 19 15:05:51 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="-0.62" x-max="5.62" y-min="-3.13" y-max="7.5" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(2.49,0);(2.49,0);(2.5,7.5);(2.5,7.5)"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,0);(5.62,0);(2.49,-3.13);(2.49,-3.13);(2.49,-3.13);(-0.62,0);
%	(-0.62,0)"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(2.5,-1.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\variable$
%</text>
%<multicurve fill-style= "none"
%	 points= "(-0.62,0);(-0.62,0);(5.62,0);(5.62,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(5.62,7.5)
\psline{->}(2.49,0)(2.5,7.5)
\psline(5.62,0)
(2.49,-3.13)(-0.62,0)
\rput(2.5,-1.25){$\variable$}
\psline(-0.62,0)(5.62,0)
\end{pspicture}


==> PIC/fp-wider-elt.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Jul 05 15:00:30 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.25" y-min="-7.5" y-max="5.63" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,0);(8.12,0);(8.12,5.63);(8.12,5.63)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,-2.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,0);(0,0);(16.25,0);(16.25,0);(16.25,0);(8.12,-7.5);
%	(8.12,-7.5);(8.12,-7.5);(0,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.25,5.63)
\psline{->}(8.12,0)(8.12,5.63)
\rput(8.12,-2.5){$\bhh$}
\pspolygon(0,0)
(16.25,0)
(8.12,-7.5)(0,0)
\end{pspicture}


==> PIC/fp-wider.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sat Jul 07 18:02:59 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.24" y-min="-12.5" y-max="12.5" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,-5);(8.12,-5);(8.12,0.63);(8.12,0.63)"
%	 />
%<parallelogram p3= "(13.74,0.75)"
%	 p2= "(13.74,6.75)"
%	 fill-style= "none"
%	 p1= "(2.5,6.75)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,6.87);(8.12,6.87);(8.12,12.5);(8.12,12.5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,3.63)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(8.12,-7.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0,-5);(0,-5);(16.24,-5);(16.24,-5);(16.24,-5);(8.12,-12.5);
%	(8.12,-12.5);(8.12,-12.5);(0,-5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.24,12.5)
\psline{->}(8.12,-5)(8.12,0.63)
\pspolygon[](2.5,6.75)(13.74,6.75)(13.74,0.75)(2.5,0.75)
\psline{->}(8.12,6.87)(8.12,12.5)
\rput(8.12,3.63){$\ahh$}
\rput(8.12,-7.5){$\bhh$}
\pspolygon(0,-5)
(16.24,-5)
(8.12,-12.5)(0,-5)
\end{pspicture}


==> PIC/inner-product-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Aug 23 14:36:15 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="16.25" y-min="6.25" y-max="29.38" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(3.12,10);(3.12,10);(3.12,15.62);(3.12,15.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,15.62);(16.25,15.62);(0,15.62);(0,15.62);(0,15.62);(5,20.62);
%	(5,20.62);(5,20.62);(11.25,20.62);(11.25,20.62);(11.25,20.62);(16.25,15.62)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(8.12,20.62);(8.12,20.62);(8.12,26.25);(8.12,26.25)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(13.12,10);(13.12,10);(13.12,15.62);(13.12,15.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,8.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(13.12,8.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.25,26.25);(11.25,26.25);(5,26.25);(5,26.25);(5,26.25);(8.12,29.38);
%	(8.12,29.38);(8.12,29.38);(8.12,29.38);(8.12,29.38);(8.12,29.38);(11.25,26.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(16.25,10);(16.25,10);(10,10);(10,10);(10,10);(13.12,6.25);
%	(13.12,6.25);(13.12,6.25);(13.12,6.25);(13.12,6.25);(13.12,6.25);(16.25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,10);(6.25,10);(0,10);(0,10);(0,10);(3.12,6.25);
%	(3.12,6.25);(3.12,6.25);(3.12,6.25);(3.12,6.25);(3.12,6.25);(6.25,10)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(16.25,29.38)
\psline{->}(3.12,10)(3.12,15.62)
\pspolygon(16.25,15.62)
(0,15.62)
(5,20.62)
(11.25,20.62)(16.25,15.62)
\psline{->}(8.12,20.62)(8.12,26.25)
\psline{->}(13.12,10)(13.12,15.62)
\rput(3.12,8.75){$\one$}
\rput(13.12,8.75){$\two$}
\pscustom[]{\psline(11.25,26.25)(5,26.25)
\psline(5,26.25)(8.12,29.38)
\psbezier(8.12,29.38)(8.12,29.38)(8.12,29.38)
\psline(8.12,29.38)(11.25,26.25)
\closepath}
\pscustom[]{\psline(16.25,10)(10,10)
\psline(10,10)(13.12,6.25)
\psbezier(13.12,6.25)(13.12,6.25)(13.12,6.25)
\psline(13.12,6.25)(16.25,10)
\closepath}
\pscustom[]{\psline(6.25,10)(0,10)
\psline(0,10)(3.12,6.25)
\psbezier(3.12,6.25)(3.12,6.25)(3.12,6.25)
\psline(3.12,6.25)(6.25,10)
\closepath}
\end{pspicture}


==> PIC/moncat-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 11:27:47 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="65" y-min="5" y-max="53" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,34)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(35,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ih$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(65,53)
\rput(5,5){$\ah$}
\rput(15,34){$\bh$}
\rput(34,53){$\ch$}
\rput(45,35){$\chh$}
\rput(65,45){$\dh$}
\rput(65,5){$\aah$}
\rput(35,5){$\ih$}
\end{pspicture}


==> PIC/moncat-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 15:16:39 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="5" y-max="53" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(15,34)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(34,53)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(45,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6,8);(6,8);(9,17);(9,17)"
%	 />
%<parallelogram p3= "(13,17)"
%	 p2= "(13,23)"
%	 fill-style= "none"
%	 p1= "(7,23)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11,23);(11,23);(13.75,31.25);(13.75,31.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,37);(17,37);(21,41);(21,41)"
%	 />
%<parallelogram p3= "(27,41)"
%	 p2= "(27,47)"
%	 fill-style= "none"
%	 p1= "(21,47)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(27,47);(27,47);(31,51);(31,51)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(24,44)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(40.62,22.5);(40.62,22.5);(44,32);(44,32)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(40,20)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,22);(65,22)"
%	 />
%<parallelogram p3= "(68,22)"
%	 p2= "(68,28)"
%	 fill-style= "none"
%	 p1= "(62,28)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,28);(65,28);(65,42);(65,42)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(65,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(36.88,22.5);(36.88,22.5);(43.75,22.5);(43.75,22.5);(43.75,22.5);(40,16.25);
%	(40,16.25);(40,16.25);(36.88,22.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53)
\rput(5,5){$\ah$}
\rput(15,34){$\bh$}
\rput(34,53){$\ch$}
\rput(45,35){$\chh$}
\rput(65,45){$\dh$}
\psline{->}(6,8)(9,17)
\pspolygon[](7,23)(13,23)(13,17)(7,17)
\psline{->}(11,23)(13.75,31.25)
\rput(10,20){$\af$}
\psline{->}(17,37)(21,41)
\pspolygon[](21,47)(27,47)(27,41)(21,41)
\psline{->}(27,47)(31,51)
\rput(24,44){$\ag$}
\psline{->}(40.62,22.5)(44,32)
\rput(40,20){$\ak$}
\psline{->}(65,8)(65,22)
\pspolygon[](62,28)(68,28)(68,22)(62,22)
\psline{->}(65,28)(65,42)
\rput(65,25){$\ahh$}
\rput(65,5){$\aah$}
\pspolygon(36.88,22.5)
(43.75,22.5)
(40,16.25)(36.88,22.5)
\end{pspicture}


==> PIC/moncat-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 11:48:49 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="5" y-max="53" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(34,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(6,8);(6,8);(9,17);(9,17)"
%	 />
%<parallelogram p3= "(13,17)"
%	 p2= "(13,23)"
%	 p1= "(7,23)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(11,23);(11,23);(22.5,40.62);(22.5,40.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(27,41)"
%	 p2= "(27,47)"
%	 p1= "(21,47)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(27,47);(27,47);(31,51);(31,51)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(24,44)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(40.62,22.5);(40.62,22.5);(44,32);(44,32)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(40,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,22);(65,22)"
%	 />
%<parallelogram p3= "(68,22)"
%	 p2= "(68,28)"
%	 p1= "(62,28)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,28);(65,28);(65,42);(65,42)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(36.88,22.5);(36.88,22.5);(43.75,22.5);(43.75,22.5);(43.75,22.5);(40,16.25);
%	(40,16.25);(40,16.25);(36.88,22.5)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53)
\rput(5,5){$\ah$}
\rput(14.38,33.75){$\bh$}
\rput(34,53){$\ch$}
\rput(45,35){$\chh$}
\rput(65,45){$\dh$}
\psline{->}(6,8)(9,17)
\pspolygon[](7,23)(13,23)(13,17)(7,17)
\psline{->}(11,23)(22.5,40.62)
\rput(10,20){$\af$}
\pspolygon[](21,47)(27,47)(27,41)(21,41)
\psline{->}(27,47)(31,51)
\rput(24,44){$\ag$}
\psline{->}(40.62,22.5)(44,32)
\rput(40,20){$\ak$}
\psline{->}(65,8)(65,22)
\pspolygon[](62,28)(68,28)(68,22)(62,22)
\psline{->}(65,28)(65,42)
\rput(65,25){$\ahh$}
\rput(65,5){$\aah$}
\pspolygon(36.88,22.5)
(43.75,22.5)
(40,16.25)(36.88,22.5)
\end{pspicture}


==> PIC/moncat-5.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Mon Jul 23 16:50:08 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.62" x-max="28" y-min="5" y-max="53.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(0.62,32.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(4,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(14.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,7.5);(5,7.5);(5,21.88);(5,21.88)"
%	 />
%<parallelogram p3= "(8,22)"
%	 p2= "(8,28)"
%	 p1= "(2,28)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,28.12);(5,28.12);(5,36.88);(5,36.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(8,37)"
%	 p2= "(8,43)"
%	 p1= "(2,43)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,43.12);(5,43.12);(5,50);(5,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(15.62,18.12);(15.62,18.12);(15.62,50);(15.62,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,15.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,8);(25,8);(25,22);(25,22)"
%	 />
%<parallelogram p3= "(28,22)"
%	 p2= "(28,28)"
%	 p1= "(22,28)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(25,28);(25,28);(25,50);(25,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(25,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(11.88,18.12);(11.88,18.12);(18.75,18.12);(18.75,18.12);(18.75,18.12);(15,11.88);
%	(15,11.88);(15,11.88);(11.88,18.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(28,53.12)
\rput(0.62,32.5){$\bh$}
\rput(4,53){$\ch$}
\rput(14.38,53.12){$\chh$}
\rput(25,53.12){$\dh$}
\psline{->}(5,7.5)(5,21.88)
\pspolygon[](2,28)(8,28)(8,22)(2,22)
\psline{->}(5,28.12)(5,36.88)
\rput(5,25){$\af$}
\pspolygon[](2,43)(8,43)(8,37)(2,37)
\psline{->}(5,43.12)(5,50)
\rput(5,40){$\ag$}
\psline{->}(15.62,18.12)(15.62,50)
\rput(15,15.62){$\ak$}
\psline{->}(25,8)(25,22)
\pspolygon[](22,28)(28,28)(28,22)(22,22)
\psline{->}(25,28)(25,50)
\rput(25,25){$\ahh$}
\rput(25,5){$\aah$}
\pspolygon(11.88,18.12)
(18.75,18.12)
(15,11.88)(11.88,18.12)
\rput(5,5){$\aah$}
\end{pspicture}


==> PIC/moncat-6.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 12:15:11 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="4.38" y-max="53.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(40.62,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,7.5);(45,7.5);(45,15.62);(45,15.62)"
%	 />
%<parallelogram p3= "(48,15.75)"
%	 p2= "(48,21.75)"
%	 p1= "(42,21.75)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,21.88);(45,21.88);(45,36.88);(45,36.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\af$
%</text>
%<parallelogram p3= "(48,37)"
%	 p2= "(48,43)"
%	 p1= "(42,43)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,43.12);(45,43.12);(45,50);(45,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ag$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55.62,48.75);(55.62,48.75);(55.62,50);(55.62,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(30,8.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,36.88);(65,36.88)"
%	 />
%<parallelogram p3= "(68,37)"
%	 p2= "(68,43)"
%	 p1= "(62,43)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,43.12);(65,43.12);(65,50);(65,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(26.88,10.62);(26.88,10.62);(33.75,10.62);(33.75,10.62);(33.75,10.62);(30,4.38);
%	(30,4.38);(30,4.38);(26.88,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(30,10.62);(30,10.62);(30,22.5);(34.38,26.25);(38.75,30);(41.88,30);
%	(45,31.25);(48.12,32.5);(50,33.75);(52.5,37.5);(55,41.25);(55.62,49.38);
%	(55.62,49.38)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53.12)
\rput(5,5){$\ah$}
\rput(40.62,25){$\bh$}
\rput(44,53){$\ch$}
\rput(54.38,53.12){$\chh$}
\rput(65,53.12){$\dh$}
\psline{->}(45,7.5)(45,15.62)
\pspolygon[](42,21.75)(48,21.75)(48,15.75)(42,15.75)
\psline{->}(45,21.88)(45,36.88)
\rput(45,18.75){$\af$}
\pspolygon[](42,43)(48,43)(48,37)(42,37)
\psline{->}(45,43.12)(45,50)
\rput(45,40){$\ag$}
\psline{->}(55.62,48.75)(55.62,50)
\rput(30,8.12){$\ak$}
\psline{->}(65,8)(65,36.88)
\pspolygon[](62,43)(68,43)(68,37)(62,37)
\psline{->}(65,43.12)(65,50)
\rput(65,40){$\ahh$}
\rput(65,5){$\aah$}
\pspolygon(26.88,10.62)
(33.75,10.62)
(30,4.38)(26.88,10.62)
\rput(45,5){$\aah$}
\pscustom[]{\psbezier(30,10.62)(30,10.62)(30,22.5)(34.38,26.25)
\psbezier(38.75,30)(41.88,30)(45,31.25)
\psbezier(48.12,32.5)(50,33.75)(52.5,37.5)
\psbezier(55,41.25)(55.62,49.38)(55.62,49.38)
}
\end{pspicture}


==> PIC/moncat-7.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 12:29:48 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68" y-min="5" y-max="53.12" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,7.5);(45,7.5);(45,22.5);(45,22.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,37.5);(45,37.5);(45,50);(45,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55.62,37.5);(55.62,37.5);(55.62,50);(55.62,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,8);(65,8);(65,22.5);(65,22.5)"
%	 />
%<parallelogram p3= "(68,22.5)"
%	 p2= "(68,37.5)"
%	 p1= "(42,37.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,37.5);(65,37.5);(65,50);(65,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,25.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(45,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\formula$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eql$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,53.12)
\rput(5,5){$\ah$}
\rput(44,53){$\ch$}
\rput(54.38,53.12){$\chh$}
\rput(65,53.12){$\dh$}
\psline{->}(45,7.5)(45,22.5)
\psline{->}(45,37.5)(45,50)
\psline{->}(55.62,37.5)(55.62,50)
\psline{->}(65,8)(65,22.5)
\pspolygon[](42,37.5)(68,37.5)(68,22.5)(42,22.5)
\psline{->}(65,37.5)(65,50)
\rput(55,25.62){$\ahh$}
\rput(65,5){$\aah$}
\rput(45,5){$\aah$}
\rput(55,33.75){$\formula$}
\rput(55,30){$\eql$}
\end{pspicture}


==> PIC/moncat-8.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 13:17:16 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="68.25" y-min="-1" y-max="55" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44,53)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ch$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(54.38,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(68.12,43.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(50,12);(50,12);(45,22.5);(45,22.5)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(45,37.5);(45,37.5);(45,50);(45,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55.62,37.5);(55.62,37.5);(55.62,50);(55.62,50)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(60,12);(60,12);(65,22.5);(65,22.5)"
%	 />
%<parallelogram p3= "(68,22.5)"
%	 p2= "(68,37.5)"
%	 p1= "(42,37.5)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(65,37.5);(65,37.5);(65,50);(65,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,25.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,-1)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,33.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\formula$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eql$
%</text>
%<multicurve fill-style= "none"
%	 points= "(47,12);(47,12);(63.25,12);(63.25,12);(63.25,12);(58.25,7);
%	(58.25,7);(58.25,7);(52,7);(52,7);(52,7);(47,12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(55,2);(55,2);(55,7);(55,7)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(55,9.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\diagonal$
%</text>
%<multicurve fill-style= "none"
%	 points= "(62,50);(62,50);(68.25,50);(68.25,50);(68.25,50);(65.12,55);
%	(65.12,55);(65.12,55);(65.12,55);(65.12,55);(65.12,55);(62,50)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(65,52)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\delete$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(65.62,16.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(44.38,16.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68.25,55)
\rput(5,5){$\ah$}
\rput(44,53){$\ch$}
\rput(54.38,53.12){$\chh$}
\rput(68.12,43.12){$\dh$}
\psline{->}(50,12)(45,22.5)
\psline{->}(45,37.5)(45,50)
\psline{->}(55.62,37.5)(55.62,50)
\psline{->}(60,12)(65,22.5)
\pspolygon[](42,37.5)(68,37.5)(68,22.5)(42,22.5)
\psline{->}(65,37.5)(65,50)
\rput(55,25.62){$\ahh$}
\rput(55,-1){$\aah$}
\rput(55,33.75){$\formula$}
\rput(55,30){$\eql$}
\pspolygon(47,12)
(63.25,12)
(58.25,7)
(52,7)(47,12)
\psline{->}(55,2)(55,7)
\rput(55,9.38){$\diagonal$}
\pscustom[]{\psline(62,50)(68.25,50)
\psline(68.25,50)(65.12,55)
\psbezier(65.12,55)(65.12,55)(65.12,55)
\psline(65.12,55)(62,50)
\closepath}
\rput(65,52){$\delete$}
\rput(65.62,16.88){$\aah$}
\rput(44.38,16.88){$\aah$}
\end{pspicture}


==> PIC/poly-diags.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 17:06:04 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="68" y-min="-9" y-max="45.07" auto-bounding="true">
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 anchor-point= "(40.75,-6)"
%	 fill-style= "none"
%	 arrow-tbar-width-linewidth-scale= "2"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(19,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\leftcat$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(49,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\rightcat$
%</text>
%<multicurve right-arrow= "head"
%	 left-arrow= "t-bar-flushed"
%	 fill-style= "none"
%	 points= "(40,22.5);(40,22.5);(28.12,22.5);(28.12,22.5)"
%	 />
%<parallelogram p3= "(57.59,26.58)"
%	 p2= "(57.59,23.16)"
%	 p1= "(44.79,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(51.19,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle h$
%</text>
%<parallelogram p3= "(63.99,12.33)"
%	 p2= "(63.99,8.91)"
%	 p1= "(54.39,8.91)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(63.99,10.62)"
%	 p2= "(63.99,10.62)"
%	 p1= "(63.99,10.62)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(62.39,5.49);(62.39,5.49);(62.39,8.91);(62.39,8.91)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(56,-9);(56,-9);(55.99,8.91);(55.99,8.91)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(55.99,12.33);(55.99,12.33);(55.99,23.16);(55.99,23.16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(59.19,10.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle g$
%</text>
%<parallelogram p3= "(63.99,26.58)"
%	 p2= "(63.99,23.16)"
%	 p1= "(59.19,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(61.59,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle f$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(59,-9);(59,-9);(59,9);(59,9)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(62.79,18.6);(62.79,18.6);(62.79,23.16);(62.79,23.16)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(47.99,26.58);(47.99,26.58);(48,36);(48,36)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(61.59,26.58);(61.59,26.58);(61.59,29.43);(61.59,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(54.39,26.58);(54.39,26.58);(54.38,35.93);(54.38,35.93)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(59.99,29.43);(59.99,29.43);(61.59,31.71);(61.59,31.71);(61.59,31.71);(63.19,29.43);
%	(63.19,29.43);(63.19,29.43);(59.99,29.43);(59.99,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(46.44,15.75);(46.44,15.75);(46.44,22.88);(46.44,22.88)"
%	 />
%<parallelogram p3= "(15.59,26.58)"
%	 p2= "(15.59,23.16)"
%	 p1= "(2.79,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(9.19,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle h$
%</text>
%<parallelogram p3= "(21.99,12.33)"
%	 p2= "(21.99,8.91)"
%	 p1= "(12.39,8.91)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<parallelogram p3= "(21.99,10.62)"
%	 p2= "(21.99,10.62)"
%	 p1= "(21.99,10.62)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(14,-9);(14,-9);(13.99,8.91);(13.99,8.91)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(13.99,12.33);(13.99,12.33);(13.99,23.16);(13.99,23.16)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(17.19,10.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle g$
%</text>
%<parallelogram p3= "(21.99,26.58)"
%	 p2= "(21.99,23.16)"
%	 p1= "(17.19,23.16)"
%	 stroke-width= "0.12"
%	 fill-style= "none"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(19.59,24.87)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle f$
%</text>
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(17,-9);(17,-9);(17,9);(17,9)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(6,26.56);(6,26.56);(6,36);(6,36)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(19.59,26.58);(19.59,26.58);(19.59,29.43);(19.59,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(12.5,26.57);(12.5,26.57);(12.5,36.02);(12.5,36.02)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(17.99,29.43);(17.99,29.43);(19.59,31.71);(19.59,31.71);(19.59,31.71);(21.19,29.43);
%	(21.19,29.43);(21.19,29.43);(17.99,29.43);(17.99,29.43)"
%	 />
%<multicurve stroke-width= "0.12"
%	 fill-style= "none"
%	 points= "(4,2);(4,2);(4,23);(4,23)"
%	 />
%<parallelogram right-arrow= "head"
%	 p3= "(26,-2)"
%	 p2= "(26,33)"
%	 p1= "(0,33)"
%	 fill-style= "none"
%	 />
%<pscurve stroke-width= "0.12"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(20,9);(20,9);(19,6);(9,7);(7,6);(6.25,4.38);
%	(6,2);(6,2);(6,2);(6.25,1.88)"
%	 />
%<pscurve stroke-width= "0.15"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(8,2);(8,2);(8.75,5);(10.71,5.39);(21,3);(23.75,6.88);
%	(21.88,15.62);(21.25,18.12);(21,20);(21,23);(21,23)"
%	 />
%<multicurve stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(6,-1);(6,-1);(6,-9);(6,-9)"
%	 />
%<pscurve right-arrow= "head"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(19,42);(19,42);(33,45);(49,42);(53,40)"
%	 />
%<pscurve right-arrow= "head"
%	 closed= "false"
%	 fill-style= "none"
%	 curvature= "1;0.1;0"
%	 points= "(48.99,38.22);(48.99,38.22);(34.92,35.59);(19,39);(15.05,41.1)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(48.97,15.86);(48.97,15.86);(46.47,13.36);(46.47,13.36);(46.47,13.36);(43.97,15.86);
%	(43.97,15.86)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(65.36,18.54);(65.36,18.54);(62.86,16.04);(62.86,16.04);(62.86,16.04);(60.36,18.54);
%	(60.36,18.54)"
%	 />
%<multicurve stroke-width= "0.05"
%	 fill-style= "solid"
%	 points= "(64.91,5.54);(64.91,5.54);(62.41,3.04);(62.41,3.04);(62.41,3.04);(59.91,5.54);
%	(59.91,5.54)"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(5.67,-6.39)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\scriptstyle X$
%</text>
%<multicurve right-arrow= "head"
%	 stroke-width= "0.15"
%	 fill-style= "none"
%	 points= "(2.05,1.98);(2.05,1.98);(10.05,1.98);(10.05,1.98);(10.05,1.98);(8.05,-1.02);
%	(8.05,-1.02);(8.05,-1.02);(4.05,-1.02);(4.05,-1.02);(4.05,-1.02);(2.05,1.98)"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(6.03,0.39)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle \Delta$
%</text>
%<parallelogram right-arrow= "head"
%	 p3= "(68,-2)"
%	 p2= "(68,33)"
%	 p1= "(42,33)"
%	 fill-style= "none"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 anchor-point= "(34.46,24.09)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\scriptstyle \kappa x.$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(68,45.07)
\rput(40.75,-6){}
\rput[r](19,40){$\leftcat$}
\rput[l](49,40){$\rightcat$}
\psline{|*->}(40,22.5)(28.12,22.5)
\pspolygon[linewidth=0.12](44.79,23.16)(57.59,23.16)(57.59,26.58)(44.79,26.58)
\rput(51.19,24.87){$\scriptstyle h$}
\pspolygon[linewidth=0.12](54.39,8.91)(63.99,8.91)(63.99,12.33)(54.39,12.33)
\pspolygon[linewidth=0.12](63.99,10.62)(63.99,10.62)(63.99,10.62)(63.99,10.62)
\psline[linewidth=0.12](62.39,5.49)(62.39,8.91)
\psline[linewidth=0.12](56,-9)(55.99,8.91)
\psline[linewidth=0.12](55.99,12.33)(55.99,23.16)
\rput(59.19,10.62){$\scriptstyle g$}
\pspolygon[linewidth=0.12](59.19,23.16)(63.99,23.16)(63.99,26.58)(59.19,26.58)
\rput(61.59,24.87){$\scriptstyle f$}
\psline[linewidth=0.12](59,-9)(59,9)
\psline[linewidth=0.12](62.79,18.6)(62.79,23.16)
\psline[linewidth=0.12](47.99,26.58)(48,36)
\psline[linewidth=0.12](61.59,26.58)(61.59,29.43)
\psline[linewidth=0.12](54.39,26.58)(54.38,35.93)
\psline[linewidth=0.12](59.99,29.43)
(61.59,31.71)
(63.19,29.43)(59.99,29.43)
\psline[linewidth=0.12](46.44,15.75)(46.44,22.88)
\pspolygon[linewidth=0.12](2.79,23.16)(15.59,23.16)(15.59,26.58)(2.79,26.58)
\rput(9.19,24.87){$\scriptstyle h$}
\pspolygon[linewidth=0.12](12.39,8.91)(21.99,8.91)(21.99,12.33)(12.39,12.33)
\pspolygon[linewidth=0.12](21.99,10.62)(21.99,10.62)(21.99,10.62)(21.99,10.62)
\psline[linewidth=0.12](14,-9)(13.99,8.91)
\psline[linewidth=0.12](13.99,12.33)(13.99,23.16)
\rput(17.19,10.62){$\scriptstyle g$}
\pspolygon[linewidth=0.12](17.19,23.16)(21.99,23.16)(21.99,26.58)(17.19,26.58)
\rput(19.59,24.87){$\scriptstyle f$}
\psline[linewidth=0.12](17,-9)(17,9)
\psline[linewidth=0.12](6,26.56)(6,36)
\psline[linewidth=0.12](19.59,26.58)(19.59,29.43)
\psline[linewidth=0.12](12.5,26.57)(12.5,36.02)
\psline[linewidth=0.12](17.99,29.43)
(19.59,31.71)
(21.19,29.43)(17.99,29.43)
\psline[linewidth=0.12](4,2)(4,23)
\pspolygon[](0,33)(26,33)(26,-2)(0,-2)
\psecurve[linewidth=0.12,curvature=1.0 0.1 0.0](20,9)(20,9)(19,6)(9,7)(7,6)(6.25,4.38)(6,2)(6,2)(6,2)(6.25,1.88)
\psecurve[linewidth=0.15,curvature=1.0 0.1 0.0](8,2)(8,2)(8.75,5)(10.71,5.39)(21,3)(23.75,6.88)(21.88,15.62)(21.25,18.12)(21,20)(21,23)(21,23)
\psline[linewidth=0.15](6,-1)(6,-9)
\psecurve{->}(19,42)(19,42)(33,45)(49,42)(53,40)
\psecurve{->}(48.99,38.22)(48.99,38.22)(34.92,35.59)(19,39)(15.05,41.1)
\psline[linewidth=0.05,fillstyle=solid](48.97,15.86)
(46.47,13.36)(43.97,15.86)
\psline[linewidth=0.05,fillstyle=solid](65.36,18.54)
(62.86,16.04)(60.36,18.54)
\psline[linewidth=0.05,fillstyle=solid](64.91,5.54)
(62.41,3.04)(59.91,5.54)
\rput[r](5.67,-6.39){$\scriptstyle X$}
\pspolygon[linewidth=0.15](2.05,1.98)
(10.05,1.98)
(8.05,-1.02)
(4.05,-1.02)(2.05,1.98)
\rput(6.03,0.39){$\scriptstyle \Delta$}
\pspolygon[](42,33)(68,33)(68,-2)(42,-2)
\rput(34.46,24.09){$\scriptstyle \kappa x.$}
\end{pspicture}


==> PIC/poly.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Sun Jul 15 16:46:34 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="3.75" x-max="52.5" y-min="0" y-max="23.12" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 left-arrow= "reverse-head"
%	 arrow-tbar-width-minimum= "0.15"
%	 fill-style= "none"
%	 points= "(5.12,13);(5.12,13);(24.12,22);(24.12,22)"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-tbar-width-minimum= "0.15"
%	 fill-style= "none"
%	 points= "(5.12,11);(5.12,11);(25.12,2);(25.12,2)"
%	 />
%<multicurve right-arrow= "head"
%	 arrow-tbar-width-minimum= "0.15"
%	 stroke-dasharray= "1;1"
%	 fill-style= "none"
%	 stroke-style= "dashed"
%	 points= "(28.12,20);(28.12,20);(28.12,3.12);(28.12,3.12)"
%	 />
%<text right-arrow= "head"
%	 text-vert-align= "center-v"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 anchor-point= "(36.12,0)"
%	 fill-style= "none"
%	 arrow-tbar-width-linewidth-scale= "2"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%
%</text>
%<multicurve right-arrow= "head"
%	 left-arrow= "t-bar-flushed"
%	 arrow-tbar-width-minimum= "0.15"
%	 fill-style= "none"
%	 points= "(51.25,20);(51.25,20);(51.25,3.12);(51.25,3.12)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(25.62,23.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Polycat$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(26.25,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Target$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,23.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\variable$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(52.5,0.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\target$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,11.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\Category$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(13.75,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Functor$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(29.38,11.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\Indfunctor$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(13.75,18.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Unit$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(52.5,23.12)
\psline[tbarsize=0.15 5]{>->}(5.12,13)(24.12,22)
\psline[tbarsize=0.15 5]{->}(5.12,11)(25.12,2)
\psline[linestyle=dashed,dash=1 1,tbarsize=0.15 5]{->}(28.12,20)(28.12,3.12)
\rput(36.12,0){}
\psline[tbarsize=0.15 5]{|*->}(51.25,20)(51.25,3.12)
\rput[l](25.62,23.12){$\Polycat$}
\rput[l](26.25,0.62){$\Target$}
\rput(52.5,23.12){$\variable$}
\rput(52.5,0.62){$\target$}
\rput[r](3.75,11.88){$\Category$}
\rput[t](13.75,5){$\Functor$}
\rput[l](29.38,11.88){$\Indfunctor$}
\rput[b](13.75,18.75){$\Unit$}
\end{pspicture}


==> PIC/program.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 17:28:12 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.13" x-max="10" y-min="-6" y-max="7" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,7)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\chh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,0);(5,0);(5,5);(5,5)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-2)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ak$
%</text>
%<multicurve fill-style= "none"
%	 points= "(0.13,0);(0.13,0);(10,0);(10,0);(10,0);(5,-6);
%	(5,-6);(5,-6);(0.13,0)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,7)
\rput(5,7){$\chh$}
\psline{->}(5,0)(5,5)
\rput(5,-2){$\ak$}
\pspolygon(0.13,0)
(10,0)
(5,-6)(0.13,0)
\end{pspicture}


==> PIC/semigroup-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 24 07:18:52 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1" x-max="65" y-min="-0" y-max="26" auto-bounding="true">
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(15,16);(15,16);(15,-0);(15,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(17,16);(17,16);(5,16);(5,16);(5,16);(8,20);
%	(8,20);(8,20);(14,20);(14,20);(14,20);(17,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(11,20);(11,20);(11,26);(11,26)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(7,16);(7,16);(7,10);(7,10)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(11,6);(11,6);(11,-0);(11,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(13,6);(13,6);(1,6);(1,6);(1,6);(4,10);
%	(4,10);(4,10);(10,10);(10,10);(10,10);(13,6)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(3,6);(3,6);(3,-0);(3,-0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(22,13)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(31,16);(31,16);(31,-0);(31,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(41,16);(41,16);(29,16);(29,16);(29,16);(32,20);
%	(32,20);(32,20);(38,20);(38,20);(38,20);(41,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(35,20);(35,20);(35,26);(35,26)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(39,16);(39,16);(39,10);(39,10)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(43,6);(43,6);(43,-0);(43,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(45,6);(45,6);(33,6);(33,6);(33,6);(36,10);
%	(36,10);(36,10);(42,10);(42,10);(42,10);(45,6)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(35,6);(35,6);(35,-0);(35,-0)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(63,16);(63,16);(63,-0);(63,-0)"
%	 />
%<multicurve right-arrow= "head"
%	 stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(65,16);(65,16);(53,16);(53,16);(53,16);(56,20);
%	(56,20);(56,20);(62,20);(62,20);(62,20);(65,16)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(59,20);(59,20);(59,26);(59,26)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(55,16);(55,16);(55,-0);(55,-0)"
%	 />
%<multicurve stroke-width= "0.22"
%	 fill-style= "none"
%	 points= "(59,16);(59,16);(59,-0);(59,-0)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(49,13)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$=$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(39,8)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(35,18)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(7,8)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(11,18)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comonoidd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(59,18)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\comontwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(65,26)
\psline[linewidth=0.22](15,16)(15,-0)
\pspolygon[linewidth=0.22](17,16)
(5,16)
(8,20)
(14,20)(17,16)
\psline[linewidth=0.22](11,20)(11,26)
\psline[linewidth=0.22](7,16)(7,10)
\psline[linewidth=0.22](11,6)(11,-0)
\pspolygon[linewidth=0.22](13,6)
(1,6)
(4,10)
(10,10)(13,6)
\psline[linewidth=0.22](3,6)(3,-0)
\rput(22,13){$=$}
\psline[linewidth=0.22](31,16)(31,-0)
\pspolygon[linewidth=0.22](41,16)
(29,16)
(32,20)
(38,20)(41,16)
\psline[linewidth=0.22](35,20)(35,26)
\psline[linewidth=0.22](39,16)(39,10)
\psline[linewidth=0.22](43,6)(43,-0)
\pspolygon[linewidth=0.22](45,6)
(33,6)
(36,10)
(42,10)(45,6)
\psline[linewidth=0.22](35,6)(35,-0)
\psline[linewidth=0.22](63,16)(63,-0)
\pspolygon[linewidth=0.22](65,16)
(53,16)
(56,20)
(62,20)(65,16)
\psline[linewidth=0.22](59,20)(59,26)
\psline[linewidth=0.22](55,16)(55,-0)
\psline[linewidth=0.22](59,16)(59,-0)
\rput(49,13){$=$}
\rput(39,8){$\comonoidd$}
\rput(35,18){$\comonoidd$}
\rput(7,8){$\comonoidd$}
\rput(11,18){$\comonoidd$}
\rput(59,18){$\comontwo$}
\end{pspicture}


==> PIC/seq-comp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Jul 04 17:09:29 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="10" y-min="-14.38" y-max="16.25" auto-bounding="true">
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-14.38);(5,-14.38);(5,-8.12);(5,-8.12)"
%	 />
%<parallelogram p3= "(8,-8.12)"
%	 p2= "(8,-2.12)"
%	 fill-style= "none"
%	 p1= "(2,-2.12)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-2.12);(5,-2.12);(5,3.75);(5,3.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-5.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,6.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<parallelogram p3= "(10,3.88)"
%	 p2= "(10,9.38)"
%	 fill-style= "none"
%	 p1= "(0,9.38)"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,9.38);(5,9.38);(5,16.25);(5,16.25)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(10,16.25)
\psline{->}(5,-14.38)(5,-8.12)
\pspolygon[](2,-2.12)(8,-2.12)(8,-8.12)(2,-8.12)
\psline{->}(5,-2.12)(5,3.75)
\rput(5,-5.12){$\ahh$}
\rput(5,6.88){$\aah$}
\pspolygon[](0,9.38)(10,9.38)(10,3.88)(0,3.88)
\psline{->}(5,9.38)(5,16.25)
\end{pspicture}


==> PIC/uni-eval-p-wide.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Aug 21 11:35:32 CEST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="1.25" x-max="20" y-min="-13.12" y-max="13.75" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17,13.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\dh$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(5,-6.25);(5,-6.25);(5,0.62);(5,0.62)"
%	 />
%<parallelogram p3= "(20,-1.25)"
%	 p2= "(20,4.75)"
%	 p1= "(2,4.75)"
%	 fill-style= "none"
%	 />
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,4.75);(17,4.75);(17,11.75);(17,11.75)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(16,1.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ahh$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(5,-8.12)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\aah$
%</text>
%<multicurve right-arrow= "head"
%	 fill-style= "none"
%	 points= "(17,-8.25);(17,-8.25);(17,-1.25);(17,-1.25)"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(17,-11.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\bhh$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.25,-6.25);(1.25,-6.25);(8.12,-6.25);(8.12,-6.25);(8.12,-6.25);(4.38,-13.12);
%	(4.38,-13.12);(4.38,-13.12);(1.25,-6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(3.75,3.12);(3.75,3.12);(6.25,3.12);(6.25,3.12);(6.25,3.12);(5,0.62);
%	(5,0.62);(5,0.62);(3.75,3.12)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(20,13.75)
\rput(17,13.75){$\dh$}
\psline{->}(5,-6.25)(5,0.62)
\pspolygon[](2,4.75)(20,4.75)(20,-1.25)(2,-1.25)
\psline{->}(17,4.75)(17,11.75)
\rput(16,1.75){$\ahh$}
\rput(5,-8.12){$\aah$}
\psline{->}(17,-8.25)(17,-1.25)
\rput(17,-11.25){$\bhh$}
\pspolygon(1.25,-6.25)
(8.12,-6.25)
(4.38,-13.12)(1.25,-6.25)
\pspolygon(3.75,3.12)
(6.25,3.12)
(5,0.62)(3.75,3.12)
\end{pspicture}


==> PIC/uni-type-Ahh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:42:12 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0" x-max="0" y-min="-5" y-max="10.62" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0,-5);(0,-5);(0,10.62);(0,10.62)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(0,10.62)
\psline(0,-5)(0,10.62)
\end{pspicture}


==> PIC/uni-type-Phh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:36:01 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.62" x-max="6.25" y-min="-16.25" y-max="10" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0.62,-10.62);(0.62,-10.62);(0.62,10);(0.62,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.25,-11.25);(1.25,-11.25);(1.25,9.38);(1.25,9.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,-11.88);(1.88,-11.88);(1.88,8.75);(1.88,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(4.38,-14.38);(4.38,-14.38);(4.38,6.25);(4.38,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,-15);(5,-15);(5,5.62);(5,5.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.12,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\spce$
%</text>
%<multicurve fill-style= "none"
%	 points= "(5,-15);(5,-15);(5,5.62);(5,5.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,-15.62);(5.62,-15.62);(5.62,5);(5.62,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,-15.62);(5.62,-15.62);(5.62,5);(5.62,5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,-16.25);(6.25,-16.25);(6.25,4.38);(6.25,4.38)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(6.25,10)
\psline(0.62,-10.62)(0.62,10)
\psline(1.25,-11.25)(1.25,9.38)
\psline(1.88,-11.88)(1.88,8.75)
\psline(4.38,-14.38)(4.38,6.25)
\psline(5,-15)(5,5.62)
\rput(3.12,0){$\spce$}
\psline(5,-15)(5,5.62)
\psline(5.62,-15.62)(5.62,5)
\psline(5.62,-15.62)(5.62,5)
\psline(6.25,-16.25)(6.25,4.38)
\end{pspicture}


==> PIC/uni-type-Phhh.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:45:40 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="0.62" x-max="6.88" y-min="-8.75" y-max="11.88" auto-bounding="true">
%<multicurve fill-style= "none"
%	 points= "(0.62,-2.5);(0.62,-2.5);(0.62,11.88);(0.62,11.88)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(3.75,3.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\spce$
%</text>
%<multicurve fill-style= "none"
%	 points= "(1.25,-3.12);(1.25,-3.12);(1.25,11.25);(1.25,11.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(1.88,-3.75);(1.88,-3.75);(1.88,10.62);(1.88,10.62)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5,-6.88);(5,-6.88);(5,7.5);(5,7.5)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(5.62,-7.5);(5.62,-7.5);(5.62,6.88);(5.62,6.88)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.25,-8.12);(6.25,-8.12);(6.25,6.25);(6.25,6.25)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(6.88,-8.75);(6.88,-8.75);(6.88,5.62);(6.88,5.62)"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(6.88,11.88)
\psline(0.62,-2.5)(0.62,11.88)
\rput(3.75,3.12){$\spce$}
\psline(1.25,-3.12)(1.25,11.25)
\psline(1.88,-3.75)(1.88,10.62)
\psline(5,-6.88)(5,7.5)
\psline(5.62,-7.5)(5.62,6.88)
\psline(6.25,-8.12)(6.25,6.25)
\psline(6.88,-8.75)(6.88,5.62)
\end{pspicture}


==> PIC/uni-type.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Jul 03 14:33:19 BST 2012
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="5" x-max="31.88" y-min="-13.12" y-max="10.62" auto-bounding="true">
%<text text-vert-align= "center-v"
%	 anchor-point= "(5,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Ah$
%</text>
%<multicurve fill-style= "none"
%	 points= "(10,-10);(10,-10);(10,10.62);(10,10.62)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(15,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eqls$
%</text>
%<multicurve fill-style= "none"
%	 points= "(25,-10.62);(25,-10.62);(25,10);(25,10)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(25.62,-11.25);(25.62,-11.25);(25.62,9.38);(25.62,9.38)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.25,-11.88);(26.25,-11.88);(26.25,8.75);(26.25,8.75)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(26.88,-12.5);(26.88,-12.5);(26.88,8.12);(26.88,8.12)"
%	 />
%<multicurve fill-style= "none"
%	 points= "(27.5,-13.12);(27.5,-13.12);(27.5,7.5);(27.5,7.5)"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(31.88,0)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Phh$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(31.88,10.62)
\rput(5,0){$\Ah$}
\psline(10,-10)(10,10.62)
\rput(15,0){$\eqls$}
\psline(25,-10.62)(25,10)
\psline(25.62,-11.25)(25.62,9.38)
\psline(26.25,-11.88)(26.25,8.75)
\psline(26.88,-12.5)(26.88,8.12)
\psline(27.5,-13.12)(27.5,7.5)
\rput(31.88,0){$\Phh$}
\end{pspicture}

